Real-time Network Intrusion Detection via Decision Transformers

Many cybersecurity problems that require real-time decision-making based on temporal observations can be abstracted as a sequence modeling problem, e.g., network intrusion detection from a sequence of arriving packets. Existing approaches like reinforcement learning may not be suitable for such cybersecurity decision problems, since the Markovian property may not necessarily hold and the underlying network states are often not observable. In this paper, we cast the problem of real-time network intrusion detection as casual sequence modeling and draw upon the power of the transformer architecture for real-time decision-making. By conditioning a causal decision transformer on past trajectories, consisting of the rewards, network packets, and detection decisions, our proposed framework will generate future detection decisions to achieve the desired return. It enables decision transformers to be applied to real-time network intrusion detection, as well as a novel tradeoff between the accuracy and timeliness of detection. The proposed solution is evaluated on public network intrusion detection datasets and outperforms several baseline algorithms using reinforcement learning and sequence modeling, in terms of detection accuracy and timeliness.

==> 0outline.tex <==
\textcolor{red}{Paper Thoughts}
\begin{itemize}
\color{blue}
\item Intrusion detection should be formulated as a sequential decision-making problem (making a sequence of decisions such as wait, flag as malicious, flag as benign for a sequence of packets coming in one by one), where Markovian property that is needed for RL may not hold. DT is the state-of-the-art method for sequential decision-making and can efficiently capture temporal patterns in input packet sequences for intrusion detection. 
\item  We want to learn from offline data that are captured during real-world network operations to circumvent the requirements of developing a simulator for online RL. DT supports offline sequence modeling and enables learning from network data that are already available.
\item  In our problem, we will leverage DT and formulate an interesting tradeoff between timeliness and accuracy of detection. Intuitively, a decision agent can decide to wait for more packets to come in before making a decision, while this may result in a delay in making a decision and potentially allow some malicious packets to go through, it could achieve better detection accuracy. In contrast, for tasks with more strict security requirements, we can make more swift detections even though they may not be as accurate.

\item add a figure, timely decision, $d_t$, to illustrate the timeliness.

\end{itemize}


==> 0table1.tex <==
% \begin{table}[]
% \centering
% \resizebox{0.49\textwidth}{!}{%
% \begin{tabular}{@{}cccccc@{}}
% \toprule
% \textbf{Model} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{ROC-AUC} \\ \midrule
% Model A & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 \\
% Model B & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 \\
% Model C & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 \\
% Model D & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 \\ \bottomrule
% \end{tabular}%
% }
% \caption{Sample Performance Table}
% \label{tab:my-table}
% \end{table}


\begin{table}[]
\centering
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{cccc}
\hline
\textbf{Model} & \textbf{Accuracy} & \textbf{Precision} & \textbf{F1-Score} \\ \hline
Model A        & 99.99             & 99.99              & 99.99             \\
Model B        & 99.99             & 99.99              & 99.99             \\
Model C        & 99.99             & 99.99              & 99.99             \\
Model D        & 99.99             & 99.99              & 99.99             \\ \hline
\end{tabular}%
}
\caption{}
\label{tab:my-table}
\end{table}

==> 0table2.tex <==
% \begin{table}[]
% \centering
% \resizebox{0.49\textwidth}{!}{%
% \begin{tabular}{cccc}
% \hline
% \textbf{Model} & \textbf{Accuracy} & \textbf{Reward} & \textbf{Process} \\ \hline
% Model A        & 99.99             & 99.99           & 99.99            \\
% Model B        & 99.99             & 99.99           & 99.99            \\
% Model C        & 99.99             & 99.99           & 99.99            \\
% Model D        & 99.99             & 99.99           & 99.99            \\ \hline
% \end{tabular}%
% }
% \caption{Sample Reward Table}
% \label{tab:my-table}
% \end{table}



\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccl}
\cline{1-7}
\textbf{Model} &
  \textbf{Accuracy} &
  \textbf{Precision} &
  \textbf{F1-Score} &
  \multicolumn{1}{l}{\textbf{Recall}} &
  \multicolumn{1}{l}{\textbf{Reward}} &
  \multicolumn{1}{l}{\textbf{Process}} &
  \textbf{} \\ \cline{1-7}
DT & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 &  \\
BC & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 &  \\
CQL & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 &  \\
DNN & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 &  \\ \cline{1-7}
\end{tabular}%
}
\caption{}
\label{tab:my-table}
\end{table*}

 
% \begin{table*}[h!]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{cccccccc}
% \hline
% \textbf{Model} &
%   \textbf{Accuracy} &
%   \textbf{Precision} &
%   \multicolumn{1}{l}{\textbf{Recall}} &
%   \textbf{F1-Score} &
%   \multicolumn{1}{l}{\textbf{ROC-AUC}} &
%   \multicolumn{1}{l}{\textbf{Reward}} &
%   \multicolumn{1}{l}{\textbf{Process}} \\ \hline
% Model A & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 \\
% Model B & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 \\
% Model C & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 \\
% Model D & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 & 99.99 \\ \hline
% \end{tabular}%
% }
% \caption{}
% \label{tab:my-table}
% \end{table*}
